A Mean-Field Description for AdS Black Hole

In this paper we find an equivalent mean-field description for asymptotically $AdS$ black hole in high temperature limit and in arbitrary dimensions. We obtain a class of mean-field potential for which the description is valid. We explicitly show that there is an one to one correspondence between the thermodynamics of a gas of interacting particles moving under a mean-field potential and an $AdS$ black hole, namely the equation of state, temperature, pressure, entropy and enthalpy of both the systems match. In $3+1$ dimensions, in particular, the mean-field description can be thought of as an ensemble of tiny interacting {\it asymptotically flat} black holes moving in volume $V$ and at temperature $T$. This motivates us to identify these asymptotically flat black holes as microstructure of asymptotically $AdS$ black holes in $3+1$ dimensions.

==> gdefn.tex <==
\newcommand{\half}{\frac{1}{2}}

%% Equation Commands

%% Special Symbols
\newcommand{\Tr}{\text{Tr}}
\newcommand{\ex}{\text{e}}
\newcommand{\vect}[1]{\vec{#1}}
\newcommand{\av}[1]{\<{#1}\>}
\newcommand{\seff}[1]{S_{\text{eff}}({#1})}



\newcommand{\reff}[1]{(\ref{#1})}

\newcommand{\eq}[1]{Eqn. (\ref{#1})}
\newcommand{\eqIn}[1]{(Eqn. \ref{#1})}

\newcommand{\fig}[1]{Fig. (\ref{#1})}
\newcommand{\figIn}[1]{(Fig. \ref{#1})}

\newcommand{\sctn}[1]{Section (\ref{#1})}
\newcommand{\sctnIn}[1]{(Section \ref{#1})}

\newcommand{\chptr}[1]{Chapter (\ref{#1})}
\newcommand{\chptrIn}[1]{(Chapter \ref{#1})}

\newcommand{\apndx}[1]{Appendix (\ref{#1})}
\newcommand{\apndxIn}[1]{(Appendix \ref{#1})}

\newcommand{\nn}{\nonumber}

\newcommand{\ben}{\begin{eqnarray}\displaystyle}
\newcommand{\een}{\end{eqnarray}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\newcommand{\bea}[1]{\begin{align}#1\end{align}}
\newcommand{\bem}[1]{\begin{multline}#1\end{multline}}
\newcommand{\bee}[1]{\begin{equation}#1\end{equation}}

\newcommand{\dbrk}{\right. \\ \left.}
\newcommand{\tbrk}{\right. \right. \\ \left. \left.}
\newcommand{\qbrk}{\right. \right. \right. \\ \left. \left. \left.}
\newcommand{\bfrac}[2]{\lb\frac{#1}{#2}\rb}

\newcommand{\dsp}{\displaystyle}

%% Text Commands

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}

%% Math Symbols

\newcommand{\grad}{{\rm {\bf \nabla}}}
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
%\newcommand{\qed}{\begin{flushright} \ensuremath{\Box} \end{flushright}}
\newcommand{\norm}[1]{|\!| #1 |\!|}

\newcommand{\df}{\mathrm{d}}

%% Symbol Shortcuts
\renewcommand{\a}{\alpha}	%%% Redefinition
\renewcommand{\b}{\beta}		%%% Redefinition
\renewcommand{\c}{\chi}		%%% Redefinition
\renewcommand{\d}{\delta}	%%% Redefinition
\newcommand{\dow}{\partial}
%\newcommand{\pa}{\partial}
\newcommand{\e}{\epsilon}
\newcommand{\ve}{\varepsilon}
\newcommand{\f}{\phi}
\newcommand{\vf}{\varphi}
\newcommand{\g}{\gamma}
\newcommand{\h}{\hbar}
\newcommand{\hs}{\hslash}
\renewcommand{\i}{\iota}		%%% Redefinition
%\renewcommand{\j}{}
\renewcommand{\k}{\kappa}	%%% Redefinition
\renewcommand{\l}{\lambda}	%%% Redefinition
\newcommand{\m}{\mu}								%%% Useless
\newcommand{\n}{\nu}								%%% Useless
\renewcommand{\o}{\omega}	%%% Redefinition
\newcommand{\p}{\psi}								%%% Useless
\newcommand{\vp}{\varpi}							%%% Useless
\newcommand{\q}{\theta}	
\newcommand{\vq}{\vartheta}	
\renewcommand{\r}{\rho}		%%% Redefinition
%\newcommand{\vr}{\varrho}	%%% Redefinition
\newcommand{\s}{\sigma}
\newcommand{\vs}{\varsigma}
\renewcommand{\t}{\tau}		%%% Redefinition
\renewcommand{\u}{\upsilon}	%%% Redefinition
%\renewcommand{\v}{}
%\newcommand{\w}{}
\newcommand{\x}{\xi}								%%% Useless
\newcommand{\bab}{\beta_{ab}}
\newcommand{\z}{\zeta}

\newcommand{\A}{\forall}
\newcommand{\B}{\Box}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\Delta}
\newcommand{\E}[1]{\mathrm{e}^{#1}}
\newcommand{\F}{\Phi}
\newcommand{\G}{\Gamma}
\newcommand{\I}{\infty}
\renewcommand{\L}{\Lambda}	%%% Redefinition
\newcommand{\M}{\mho}
\newcommand{\N}{\nabla}
\renewcommand{\O}{\Omega}	%%% Redefinition
\renewcommand{\P}{\Psi}		%%% Redefinition		%%% Useless
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\Theta}
\renewcommand{\S}{\Sigma}	%%% Redefinition
\newcommand{\U}{\Upsilon}
\newcommand{\X}{\Xi}								%%% Useless
\newcommand{\Z}{\mathcal{Z}}

%% Caligraphy
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%% Mathfrak
\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fZ}{\mathfrak{Z}}
\newcommand{\fa}{\mathfrak{a}}
\newcommand{\fb}{\mathfrak{b}}
\newcommand{\fc}{\mathfrak{c}}
\newcommand{\fd}{\mathfrak{d}}
\newcommand{\fe}{\mathfrak{e}}
\newcommand{\ff}{\mathfrak{f}}
\newcommand{\fg}{\mathfrak{g}}
\newcommand{\fh}{\mathfrak{h}}
\newcommand{\fii}{\mathfrak{i}}		%%% Out of Order
\newcommand{\fj}{\mathfrak{j}}
\newcommand{\fk}{\mathfrak{k}}
\newcommand{\fl}{\mathfrak{l}}
\newcommand{\fm}{\mathfrak{m}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fo}{\mathfrak{o}}
\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\fr}{\mathfrak{r}}
\newcommand{\fs}{\mathfrak{s}}
\newcommand{\ft}{\mathfrak{t}}
\newcommand{\fu}{\mathfrak{u}}
\newcommand{\fv}{\mathfrak{v}}
\newcommand{\fw}{\mathfrak{w}}
\newcommand{\fx}{\mathfrak{x}}
\newcommand{\fy}{\mathfrak{y}}
\newcommand{\fz}{\mathfrak{z}}

%% Standard Functions
\newcommand{\sech}{\mathrm{sech}}
\newcommand{\csch}{\mathrm{csch}}
\newcommand{\sina}[1]{\sin\lb #1 \rb}
\newcommand{\cosa}[1]{\cos\lb #1 \rb}
\newcommand{\tana}[1]{\tan\lb #1 \rb}
\newcommand{\cota}[1]{\cot\lb #1 \rb}
\newcommand{\seca}[1]{\sec\lb #1 \rb}
\newcommand{\csca}[1]{\csc\lb #1 \rb}
\newcommand{\loga}[1]{\log\lb #1 \rb}
\newcommand{\lna}[1]{\ln\lb #1 \rb}

%% Symbols
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\nra}{\nrightarrow}
\newcommand{\nRa}{\nRightarrow}
\newcommand{\lB}{\left [}
\newcommand{\rB}{\right ]}
\newcommand{\lb}{\left (}
\newcommand{\rb}{\right )}
\newcommand{\lbr}{\left \{}
\newcommand{\rbr}{\right \}}
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}		%%% Redefinition
\newcommand{\ld}{\left.}
\newcommand{\rd}{\right.}



\newcommand{\Rp}{R'(0)}

\newcommand{\vro}{\varrho}
\newcommand{\vt}{\vartheta}
\newcommand{\type}[1]{$\mathbb{Type \ #1}$}
\newcommand{\tp}[1]{$\mathbb{T#1}$}

\newcommand{\class}[1]{$\mathbb{Class \ #1}$}
\newcommand{\cl}[1]{$\mathbb{C#1}$}

\newcommand{\ds}{Dyson-Schwinger}


\newcommand{\hp}{h_{+}(\theta)}
\newcommand{\hmm}{h_{-}(\theta)}
\newcommand{\hptx}{$h_{+}(\theta)$}
\newcommand{\hmt}{$h_{-}(\theta)$}

\newcommand{\ads}{{\it AdS}}



\newcommand{\T}[{1}]{T^{#1}}
\newcommand{\Tmn}{T^{\m\n}}
\newcommand{\tc}{\theta_{\x}}



\def\Xint#1{\mathchoice
{\XXint\displaystyle\textstyle{#1}}%
{\XXint\textstyle\scriptstyle{#1}}%
{\XXint\scriptstyle\scriptscriptstyle{#1}}%
{\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
\!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$ }
\vcenter{\hbox{$#2#3$ }}\kern-.6\wd0}}
\def\ddashint{\Xint=}
\def\dashint{\Xint-}
